You Only Click Once: Single Point Weakly Supervised 3D Instance Segmentation for Autonomous Driving

Outdoor LiDAR point cloud 3D instance segmentation is a crucial task in autonomous driving. However, it requires laborious human efforts to annotate the point cloud for training a segmentation model. To address this challenge, we propose a YoCo framework, which generates 3D pseudo labels using minimal coarse click annotations in the bird's eye view plane. It is a significant challenge to produce high-quality pseudo labels from sparse annotations. Our YoCo framework first leverages vision foundation models combined with geometric constraints from point clouds to enhance pseudo label generation. Second, a temporal and spatial-based label updating module is designed to generate reliable updated labels. It leverages predictions from adjacent frames and utilizes the inherent density variation of point clouds (dense near, sparse far). Finally, to further improve label quality, an IoU-guided enhancement module is proposed, replacing pseudo labels with high-confidence and high-IoU predictions. Experiments on the Waymo dataset demonstrate YoCo's effectiveness and generality, achieving state-of-the-art performance among weakly supervised methods and surpassing fully supervised Cylinder3D. Additionally, the YoCo is suitable for various networks, achieving performance comparable to fully supervised methods with minimal fine-tuning using only 0.8% of the fully labeled data, significantly reducing annotation costs.

==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/3_method.tex <==
\section{Method}
\label{sec:method}
% 我们的目标是缩小click-level弱监督和全监督算法间的性能差距，如何生成高质量的伪标签是一个关键问题。
% Our goal is to narrow the performance gap between click-level weakly supervised and fully supervised algorithms. Generating high-quality pseudo-labels is key to achieving this.
Our goal is to generate high-quality 3D instance pseudo labels using sparse click-level annotations, and to narrow the performance gap between weakly supervised and fully supervised methods. To achieve this, we propose a simple yet effective framework, \textbf{YoCo}, which integrates pseudo label generation with network training, as illustrated in Figure \ref{fig:framework}. By leveraging the minimal input of click annotations, YoCo efficiently creates reliable pseudo labels that maintain strong performance, even with limited supervision. The detailed process is outlined as follows:

For pseudo label generation in Figure \ref{fig:framework}(a), given a set of calibrated images and point cloud data, we first annotate the point cloud with click-level labels in the BEV plane. These labels are then projected onto the corresponding images, and processed by our proposed VFM-PLG module. The VFM-PLG leverages the VFMs and geometric constraints from the point cloud to generate high-quality 3D pseudo labels, as described in Section \ref{sec:module_1}.

For network training in Figure \ref{fig:framework}(b), we adopt the MeanTeacher~\cite{tarvainen2017meanteacher} method, which involves a student network and a teacher network. The teacher network is updated using an exponential moving average (EMA) of the student’s weights. It predicts labels from adjacent frames, and the TSU module uses these predictions to refine the 3D pseudo labels generated by the VFM-PLG. This refinement incorporates temporal and spatial information from adjacent frames, as detailed in Section \ref{sec:module_2}. 

Additionally, to further boost the reliability of the pseudo labels, we introduce the ILE module. This module enhances the labels offline by using high-confidence and high-IoU results to update the 3D pseudo labels, further improving the performance of our method, as outlined in Section \ref{sec:module_3}.
% To leverage the robustness capability of neural networks, we employ the Mean Teacher framework during training. This setup consists of a student network and a teacher network, where the teacher is updated using an exponential moving average (EMA) of the student’s weights. The teacher network predicts labels from adjacent frames, and our TSU module refines the pseudo 3D labels generated by the VFM-PLG. This refinement incorporates temporal and spatial information from nearby frames, enhancing label quality.
% Additionally, to further boost the reliability of the pseudo labels, we introduce the ILE module. This module enhances the labels offline by using high-confidence scores and Intersection-over-Union (IoU) values to update the pseudo 3D labels, further improving the accuracy of our method.

\subsection{Preliminary}
\label{sec:prelimiinary}
Given a set of calibrated images and point cloud data, we utilize sensor calibration to project the point cloud onto the images, establishing a mapping relationship between the 3D points and image pixels. Specifically, consider a set of points $\mathbf{P}^{3\mathbf{d}}=\left\{ p_{i}^{3d} \right\} _{i=1}^{N}=\left\{ \left( x_i,y_i,z_i \right) \right\} _{i=1}^{N} \in \mathbb{R}^{N\times 3}$ we can obtain the corresponding pixel coordinates $\mathbf{P}^{2\mathbf{d}}=\left\{ p_{i}^{2d} \right\} _{i=1}^{N}=\left\{ \left( u_i,v_i \right) \right\} _{i=1}^{N} \in \mathbb{R}^{N\times 2}$ by applying the projection transformation formula:
\begin{equation}
\label{eq:project}
    z_c\left( u_i,v_i,1 \right) ^T=\mathbf{M}_{int}\times \mathbf{M}_{ext}\times \left( x_i,y_i,z_i,1 \right) ^T
\end{equation}
where $N$ is the number of the points, $z_c$ represents the depth of the point in the camera coordinate system, $\mathbf{M}_{int}$ and $\mathbf{M}_{ext}$ denote the intrinsic and extrinsic parameters of the camera, respectively.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.95\linewidth]{img/sam4cyc.pdf}
    \vspace{-2mm}
    % 同一个实例使用不同的Prompt（图中不同颜色的五角星）生成的2DMask的结果对比。w/o表示不结合DAM，w 表示结合DAM，使用DAM模型在不同Prompt下获得了更一致且更准确的结果。
    % Our VFM-PLG for the composite categories.
    \caption{\textbf{Our VFM-PLG for the Composite Categories.} Comparison of 2D mask results for the same instance with different prompts (colored stars). \textit{w/o} shows results without DAM, while \textit{w} shows results with DAM. Using the DAM model yields more consistent and accurate results across different prompts.}
    \vspace{-1mm}
    \label{fig:sam4cyc}
\end{figure}

\subsection{VFM-Based Pseudo Label Generation}
\label{sec:module_1}
SAM~\cite{kirillov2023segment} is a vision foundation model that inputs images and prompts to generate corresponding 2D masks. The prompts include points, bounding boxes, masks, and texts. By leveraging the projection relationship described in Equation \ref{eq:project}, we can project the click-level annotations of point clouds onto the image as prompts to obtain the object's 2D mask. Points projected within this 2D mask region can be considered the 3D pseudo label. This process can be formally expressed by the following equation:
\begin{equation}
\label{eq:color}
    m_i = Color(SAM(I_i,p_i,c_i))
\end{equation}
where $m_i$ denotes the 3D pseudo label to the $i$-th click annotation, \textit{Color} represents the operation of mapping a 2D mask to a 3D pseudo label, $I_i$, $p_i$, and $c_i$ represent the image, 2D coordinate, and the class label corresponding to the $i$-th click annotation, respectively.
% 最后一个是，在BEV平面下，由于缺少高度信息，当前click可能存在多个对应的3D点，错误的prompt将会导致错误的分割结果

However, this approach faces three challenges. First, SAM struggles with segmenting composite categories like cyclists. The second one is inaccuracies in the SAM segmentation mask and the projection relationship. Finally, due to the lack of height information in the BEV plane, there may be multiple corresponding 3D points in the current click, and an incorrect prompt will result in an inaccurate segmentation result.

To address the first issue, we utilize the Depth Anything Model (DAM)~\cite{yang2024depthanythin} as an auxiliary tool to perform depth-based smoothing, particularly for composite categories like cyclists (as shown in Figure \ref{fig:sam4cyc}).
% 具体来说，图片被送入DAM获得深度图，然后使用深度图的特征与prompt进行交互，得到对应的2D掩码
Specifically, the image is processed through the DAM to generate a depth map, and the depth map's features are then used to interact with the prompt's features, resulting in the corresponding 2D mask. (as shown in Figure \ref{fig:vfm-plg}). Therefore, Equation \ref{eq:color} is updated as:
\begin{equation}
\label{eq:color2}
    % m_i=\left\{ \begin{array}{l}
    % 	Color\left( SAM\left( I_i,p_i,c_i \right) \right)\\
    % 	Color\left( SAM\left( DAM\left( I_i \right) ,p_i,c_i \right) \right)\\
    % \end{array} \right.
    m_i= Color\left( SAM\left( DAM\left( I_i \right) ,p_i,c_i \right) \right)
\end{equation}

\begin{figure}[ht]
    \centering
    \includegraphics[width=1.0\linewidth]{img/VFM-PLG-V2.pdf}
    \caption{\textbf{Overview of VFM-PLG Module.} The blue dashed line indicates that if the generated 3D mask does not satisfy geometric constraints, another point is selected as the prompt. \textit{GC} denotes that the point cloud is processed using geometric constraints.}
    \label{fig:vfm-plg}
    \vspace{-3mm}
\end{figure}

As for the last two issues, point cloud geometric constraints are proposed for filtering the labels. Specifically, we first obtain a 3D pseudo label $m_i$ for the $i$-th object through the projection relationship. Then a clustering algorithm is applied to $m_i$, resulting in a set of clusters. The cluster containing the click annotation $p_i$ is identified as the 3D pseudo label for that object ($Find$ operation in Equation \ref{eq:filter}).
Next, a geometric consistency check is performed on the identified cluster ($Filter$ operation in Equation \ref{eq:filter}). The label is retained if the cluster satisfies certain geometric conditions; otherwise, the pseudo label is discarded, \ie, $m_i=\left\{0\right\}^N_{i=1}$. This process can be represented as follows:

\begin{equation}
\label{eq:filter}
    \tilde{m}_i=Filter\left( Find\left( Cluster\left( m_i \right) \right) \right)
\end{equation}

If the current click corresponds to multiple points, we iterate to select one as the prompt. If the current result meets the geometric constraints, it is retained as the 3D pseudo label; otherwise, a new point is re-selected as the prompt to generate the pseudo label, as indicated by the blue dashed line in Figure \ref{fig:vfm-plg}.

% 若当前click对应多个点，我们遍历选择一个作为prompt，若当前的结果满足几何约束则保留作为伪标签，否则我们重新选择一个点作为prompt来生成伪标签，如图3蓝色虚线所示。

\subsection{Temporal and Spatial-Based Label Updating}
\label{sec:module_2}
To improve the quality of pseudo labels generated by the VFM-PLG module, we propose the temporal and spatial-based label updating module. This module leverages the generalization of neural networks by using high-reliability predictions from adjacent frames to update the pseudo labels of the current frame online.

To transform the point clouds from adjacent frames to the current frame, a coordinate system transformation is required, which can be expressed by the following equation:
\begin{equation}
\label{eq:transform}
    \mathbf{P}_t=\mathbf{T}_{t}^{-1}\times \mathbf{T}_{adj}\times \mathbf{P}_{adj}
\end{equation}
where $\mathbf{T}_{t}$ is the ego-car pose in the current frame, $\mathbf{T}_{adj}$ is the ego-car pose in the adjacent frame, $\mathbf{P}_t$ and $\mathbf{P}_{adj}$ correspond to the coordinates of the point cloud in the current frame and the adjacent frame, respectively.

Unlike MWSIS's~\cite{jiang2024mwsis} PVC module, our method does not require establishing a voting space from the previous training epochs, which reduces memory requirements during training. Moreover, since it is difficult to establish a one-to-one correspondence between point clouds of adjacent frames, we employ a voxel voting mechanism. An online voxel voting space $S$ is set up, where each voxel updates its corresponding label according to a predefined update strategy. The current frame requires voxelization of the point cloud, and the updated labels are obtained from the corresponding voxel space. The specific update strategy is as follows:
\begin{itemize}
    \item \textbf{Soft voting strategy.} Consider a voxel that contains $n$ points, where each point $p_i^v$ has an associated classification confidence scores $s^v_i \in \mathbb{R}^{num}$, where the $num$ denotes the class number. We average the classification confidence scores for all points within the voxel, and then identify the class $c^v_i$ with the highest score. If this score exceeds a set threshold $T_{s}$, the class is assigned as the voxel's label. The above process can be represented by Equation \ref{eq:softvoting}. Unlike the method of directly selecting the class with the most points, this approach enhances robustness against prediction noise.
    \begin{equation}
    \label{eq:softvoting}
        c_{i}^{v}=\begin{cases}
        	\text{arg}\max \bar{s}&		\text{if\,\,}\max \bar{s} >T_s\\
        	-1&		\text{otherwise}\\
        \end{cases}
    \end{equation}
    where $\bar{s}= \frac{1}{n}\sum_{i=1}^{n}{s_{i}^{v}}$, $-1$ denotes the ignored label.
    \item \textbf{Distance-based reliability update strategy.} To improve the reliability of voting labels, we consider that a greater number of voxel points and higher point confidence result in more reliable voting. Given that LiDAR point clouds are dense near the sensor and sparse farther away, we dynamically adjust the voting threshold: voxels closer to the sensor require more votes and higher confidence for label assignment.
\end{itemize}
By applying the aforementioned update strategy, a reliable voxel voting space $S$ is constructed, which is then used to update the labels of the current frame. For further details, refer to Algorithm \ref{alg:tsu} in the supplementary material.

\begin{table*}[ht]
  \centering
  % add the adjustbox
  \adjustbox{max width=1.0\textwidth}{
    \begin{tabular}{ccccccccccc} 
    \toprule
    \multirow{2}{*}{Supervision} & \multirow{2}{*}{Annotation} & \multirow{2}{*}{Model} & \multicolumn{4}{c}{3D Instance Segmentation (AP)}        & \multicolumn{4}{c}{3D Semantic Segmentation (IoU)}            \\ 
    \cline{4-11}
                                 &                             &                        & mAP   & Veh.  & Ped.  & Cyc.  & mIoU   & Veh.   & Ped.   & Cyc.    \\ 
    \hline
    \multirow{3}{*}{Full}        & 3D Mask                     & Cylinder3D~\cite{zhu2021cylindrical}             & 51.40 & 75.31 & 38.12 & 40.76 & 78.903 & 96.476 & 83.666 & 56.567  \\
                                 & 3D Mask                     & PTv3~\cite{wu2024ptv3}                   & 60.08 & 75.73 & 53.63 & 51.32 & 83.679 & 96.686 & 85.500 & 68.852  \\
                                 & 3D Mask                     & SparseUnet~\cite{shi2020PartA2}             & 59.26 & 80.25 & 56.95 & 40.59 & 79.505 & 96.675 & 81.906 & 59.933  \\ 
    \arrayrulecolor{black}\cline{1-1}\arrayrulecolor{black}\cline{2-11}
    \multirow{9}{*}{Weak}        & 3D Box                      & SparseUnet~\cite{shi2020PartA2}             & 49.32 & 69.00 & 45.96 & 33.01 & 72.545 & 89.471 & 73.581 & 54.582  \\
                                 & 2D Box                      & SparseUnet~\cite{shi2020PartA2}             & 35.48 & 44.54 & 36.84 & 25.08 & 63.831 & 74.102 & 72.113 & 45.278  \\
                                 & 2D Box$^*$                      & SparseUnet~\cite{shi2020PartA2}             & 45.12 & 64.06 & 40.06 & 31.23 & 75.571 & 93.418 & 77.982 & 55.312  \\
                                 & 2D Box                      & MWSIS~\cite{jiang2024mwsis}                  & 48.42 & 61.45 & 45.23 & 38.59 & 75.898 & 90.369 & 78.996 & 58.329  \\
                                 & Click$^*$                       & SparseUnet~\cite{shi2020PartA2}             & 40.19 & 59.15 & 36.98 & 24.45 & 67.510 & 76.225 & 76.118 & 50.187  \\ 
    \cline{2-11}
                                 & Click$^\dag$                       & Cylinder3D~\cite{zhu2021cylindrical}             & 45.12 & 60.72 & 36.52 & 38.11 & 70.068 & 76.653 & \underline{79.123} & 54.428  \\
                                 & Click$^\dag$                       & PTv3~\cite{wu2024ptv3}                   & 46.59 & 62.59 & 38.12 & \underline{39.06} & \underline{72.776} & \textbf{82.109} & 77.056 & \underline{59.163}  \\
                                 & Click$^\dag$                      & SparseUnet~\cite{shi2020PartA2}             & \underline{47.37} & \underline{64.10} & \underline{41.50} & 36.51 & 72.189 & 79.850 & 78.619 & 58.097  \\ 
    \cline{2-11}
                                 & Click$^\dag$\cellcolor{lightgray}  & \textbf{YoCo (Ours)}\cellcolor{lightgray} & \textbf{55.35}\cellcolor{lightgray} & \textbf{67.69}\cellcolor{lightgray} & \textbf{55.25}\cellcolor{lightgray} & \textbf{43.12}\cellcolor{lightgray} & \textbf{74.770}\cellcolor{lightgray} & \underline{81.136}\cellcolor{lightgray} & \textbf{81.716}\cellcolor{lightgray} & \textbf{64.459}\cellcolor{lightgray}  \\
    \bottomrule
    \end{tabular}
  }
  \caption{\textbf{Performance Comparisons of 3D Instance and Semantic Segmentation on Waymo Validation Dataset.} The PLG denotes our proposed VFM-PLG module. Abbreviations: vehicle (Veh.), pedestrian (Ped.), cyclist (Cyc.). \textbf{Bold} indicates optimal performance, and \underline{underline} indicates sub-optimal performance. $^*$ represents the pseudo label generated by SAM using the corresponding annotation as the prompt. $^\dag$ denotes the pseudo label generated by our VFM-PLG module.}
  \vspace{-2mm}
  \label{tab:main results}
\end{table*}

\subsection{IoU-Guided Label Enhancement}
\label{sec:module_3}
To further leverage the robustness of neural networks and correct the erroneous pseudo labels generated by the VFM-PLG, we introduce an IoU-guided label enhancement module. This module performs an offline update of pseudo labels using high-confidence scores and high-IoU value predictions. Additionally, we adjust the confidence score threshold accordingly to accommodate the characteristic density variation in LiDAR point clouds (dense near, sparse far). The process can be represented as follows:
\begin{equation}
    m'_i=\begin{cases}
        \text{arg}\max \left( IoU_i \right)&		\,\,\text{if\,\,}s_i\ge T_{s_2}\,\,\text{and\,\,}IoU_i\ge T_{IoU}\\
        \tilde{m}_i&		\,\,\text{otherwise\,\,}\\
    \end{cases}
\end{equation}
where $IoU_i=\frac{\tilde{m}_i\cap \hat{m}_i}{\tilde{m}_i\cup \hat{m}_i}$, $m'_i$ and $\hat{m}_i$ represent the updated labels and the predicted labels, respectively, while $T_{s_2}$ and $T_{IoU}$ correspond to the predefined confidence scores threshold and IoU threshold.

\subsection{Loss}
\label{sec:loss}
The overall loss function of the YoCo is defined as:
\begin{equation}
    L = \alpha_1 L_{cls} + \alpha_2 L_{vote}
\end{equation}
where $L_{cls}$ denotes the cross entropy loss or focal loss, and $L_{vote}$ represents the L1 loss, $\alpha_1$ and $\alpha_2$ are hyperparameters to balance loss terms.




==> sec/4_experiment.tex <==


\section{Experiments}
\label{sec:experiment}
\subsection{Waymo Open Dataset}
% 我们遵循MWSIS论文的设置，在Waymo1.4.0数据集上进行实验
Following the state-of-the-art MWSIS~\cite{jiang2024mwsis}, we conduct our experiments on version 1.4.0 of the Waymo Open Dataset (WOD)~\cite{sun2020waymo}, which includes both well-synchronized and aligned LiDAR points and images. The WOD consists of 1,150 sequences (over 200K frames), with 798 sequences for training, 202 sequences for validation, and 150 sequences for testing. For the 3D segmentation task, the dataset contains 23,691 and 5,976 frames for training and validation, respectively. We specifically focus on the vehicle, pedestrian, and cyclist categories for evaluation.

\subsection{Implementation Details}
\noindent\textbf{Click Setting.} For the click annotation, we use the average coordinates of each instance from the BEV plane as a reference, and then select the nearest point to simulate the manual click. Meanwhile, in Table 2, we also simulate the results under different disturbance ranges.

\noindent\textbf{Evaluation Metric.} We adopt the same evaluation metrics as~\cite{jiang2024mwsis}. For 3D instance segmentation, we use average precision (AP) across different IoU thresholds to assess performance, while for 3D semantic segmentation, we use mean intersection-over-union (mIoU) as the evaluation metric.

\noindent\textbf{Training Setting.} 
% 我们选择了几种经典的backbone，如 Cylinder3D，SparseUnet, Point Transformer V3 (PTV3), and then employ two separate heads to predict semantic masks and group pixels to instances. We train Cylinder3D for 40 epochs, SparseUnet for 24 epochs, and PTV3 for 40 epochs. 所有模型都在4张3090上训练，with a batch size of 8，且采用AdamW优化器。
We choose several classic backbones, including Cylinder3D~\cite{zhu2021cylindrical}, SparseUnet~\cite{shi2020PartA2}, and Point Transformer V3 (PTv3)~\cite{wu2024ptv3}, and use two separate heads: one for predicting semantic masks and another for grouping pixels into instances. Cylinder3D, PTv3, and SparseUnet are trained for 40, 50, and 24 epochs, respectively. All models are trained on 4 NVIDIA 3090 GPUs with a batch size of 8, using the AdamW~\cite{loshchilov2017adamw} optimizer.

\subsection{Results on WOD}
% 在表格1中我们使用不同的模型进行实验，同时考虑时间和内存效率，我们选择SparseUnet作为baseline开展实验，SparseUnet对比PTv3方法拥有更快的训练速度和更低的显存需求，且有相似的性能。我们将YoCo与其他全监督和弱监督方法进行对比，在3D实例分割任务上，我们的方法对比基于其他弱监督的方法取得最佳性能，对比基于Click+SAM的方法，我们的方法提高了15.16% mAP，同时，对比标注成本更大的3D框，我们的方法提升了6.03% mAP。除此之外，我们的方法对比基于Cylinder3D的全监督的方法获得了3.95% mAP的提升。除此之外，我们还提供了3D语义分割的指标。对比基于Click+SAM的方法，我们的方法获得7.260% mIoU提升，与基于3D框的方法对比，我们实现了2.225% mIoU提升，并达到全监督性能的94.76%。
\noindent\textbf{Baseline.} In Table \ref{tab:main results}, we present experiments conducted with various models. Considering both computational time and memory efficiency, we select SparseUnet~\cite{shi2020PartA2} as the baseline for our experiments. SparseUnet, in comparison to the state-of-the-art PTv3~\cite{wu2024ptv3} method, offers several advantages: it delivers faster training times and requires significantly less memory while achieving a similar level of performance. This makes SparseUnet a more practical choice for the network without compromising on performance. 

\noindent\textbf{3D Segmentation.} We compare the YoCo with other weakly-supervised and fully-supervised methods for 3D instance segmentation. Our YoCo achieves the best performance among weakly supervised methods. It outperforms the Click+SAM-based approach with a 15.16\% improvement in mAP and surpasses the state-of-the-art method MWSIS by 6.93\% mAP, while utilizing more cost-effective sparse click annotations. Additionally, compared with methods using 3D bounding boxes, which have higher annotation costs, our approach achieves a 6.03\% mAP improvement. Moreover, our method outperforms fully-supervised methods based on Cylinder3D by 3.95\% mAP.

We also provide metrics for 3D semantic segmentation. Compared to the Click+SAM-based method, our approach achieves a 7.260\% improvement in mIoU. When compared to methods based on 3D bounding boxes, it achieves a 2.225\% mIoU increase. Additionally, our method reaches 94.76\% of the fully supervised performance.

% In Figure 5, we provide a visual comparison, and our YoCo achieves better results in some cases.

\begin{table}[ht]
    \centering
    \adjustbox{max width=0.75\linewidth}{
    \begin{tabular}{ccccc} 
    \toprule
    \multicolumn{3}{c}{Method}                 & \multirow{2}{*}{mAP}      & \multirow{2}{*}{mIoU}       \\ 
    \cline{1-3}
    VFM-PLG          & TSU          & ILE          &                           &                             \\ 
    \hline
    $\mbox{-}$   & $\mbox{-}$   & $\mbox{-}$   & \multicolumn{1}{l}{25.36} & \multicolumn{1}{l}{51.919}  \\
    \hline
    $\checkmark$ & $\mbox{-}$   & $\mbox{-}$   & 47.37                     & 72.189                      \\
    $\checkmark$ & $\checkmark$ & $\mbox{-}$   & 52.18                     & 74.449                      \\
    $\checkmark$\cellcolor{lightgray} & $\checkmark$\cellcolor{lightgray} & $\checkmark$\cellcolor{lightgray} & \textbf{55.35}\cellcolor{lightgray}            & \textbf{74.770}\cellcolor{lightgray}             \\
    \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Ablation Study of All Modules.}}
    \label{tab:ile}
    \vspace{-3mm}
\end{table}

\subsection{Ablation Study and Analysis}
\label{sec:ablation}

\noindent\textbf{Effect of all modules.}
% 表格5提供我们提出的所有模块的消融实验，当仅使用VFM-PLG模块时，性能提升明显，实例分割和语义分割性能分别提升22.01%mAP和20.27%mIoU，这证明结合VFM和点云的几何约束进行伪标签生成是一种有效的方法。当引入基于时间和空间的标签更新策略后，性能进一步提升4.81%mAP和2.26%mIoU，这表明利用神经网络的泛化能力将相邻帧的预测信息作为更新标签可以进一步的提高标签质量。除此之外，我们提出的ILE策略进一步的利用该泛化能力，对VFM-PLG生成的伪标签进行离线增强，提升标签质量，实例分割和语义分割性能分别提高了3.17%mAP，0.321%mIoU.
Table \ref{tab:ile} presents the ablation study of all the proposed modules. When solely the VFM-PLG module is utilized, we observe a substantial performance improvement, with instance segmentation and semantic segmentation improving by 22.01\% mAP and 20.270\% mIoU, respectively. This demonstrates the effectiveness of generating pseudo labels by combining the VFM module with geometric constraints from point clouds. When the TSU module is introduced, the performance further improves by 4.81\% mAP and 2.26\% mIoU. This highlights the value of leveraging the neural network’s generalization by using high-confidence predictions from adjacent frames to update the current frame’s labels,  improving the quality of the pseudo labels. Moreover, our proposed ILE module leverages the robustness of the network to perform offline refinement of the pseudo labels generated by the VFM-PLG. This approach leads to additional gains in label quality, with instance segmentation improving by 3.17\% mAP and semantic segmentation by 0.321\% mIoU. These results demonstrate the effectiveness of our framework in progressively refining pseudo labels and narrowing the performance gap between weakly supervised and fully supervised methods.



\noindent\textbf{Effect of the VFM-PLG.}
% 图2展示了我们方法可以生成高质量的伪标签，与与仅使用点击提示的方法相比，我们的VFM-PLG模块实现了近10％的性能提升。
% 图片2展示了我们方法在生成伪标签上的优越性能，在表2中，我们提供了VFM-PLG模块的消融实验。表格2的第二行表示baseline性能，仅仅使用Click和SAM得到的伪标签进行训练。仅仅使用聚类算法处理，mAP提升了14.83%。如果进一步的使用DAM对组合类别，如Cylist进行处理，使其性能提升5.82%AP。当结合几何约束(GC)时，我们将性能mAP提高到47.37%，超过了使用2D Box作为prompt的方法。通过结合上述的方法，我们大大降低了标注成本。
Figure \ref{fig:miou} demonstrates the effectiveness of our method in generating high-quality pseudo labels, and our VFM-PLG module achieves nearly a 10\% performance improvement compared to the method that uses only clicks as prompts. 
\begin{figure}[ht]
    \centering
    \includegraphics[width=1.0\linewidth]{img/miou.pdf}
    \vspace{-6mm}
    \caption{\textbf{Comparisons of IoU on WOD Validation Dataset.} We combine click-level and 2D bounding box-level annotations with various methods to generate pseudo labels for the validation dataset and evaluate them with ground truth.}
    \label{fig:miou}
    \vspace{-1mm}
\end{figure}

\begin{table}[ht]
    \centering
    \adjustbox{max width=0.7\linewidth}{
    \begin{tabular}{cccc}
    \toprule
    \multirow{2}{*}{Annotation~} & \multirow{2}{*}{Method} & \multicolumn{2}{c}{AP}           \\ 
    \cline{3-4}
                                 &                         & mAP            & Cyc.            \\ 
    \hline
    2D Box                       & SAM                     & 45.12          & 31.23           \\ 
    \hline
    \multirow{4}{*}{Click}       & SAM                     & 25.36          & 16.42           \\
                                 & + Cluster               & 40.19          & 24.45           \\
                                 & + DAM                   & 42.13          & 30.27           \\
                                 & + GC\cellcolor{lightgray}                    & \textbf{47.37}\cellcolor{lightgray} & \textbf{36.51}\cellcolor{lightgray}  \\
    \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Ablation Study for VFM-PLG Module.}}
    \label{tab:plg}
    \vspace{-3mm}
\end{table}
In Table \ref{tab:plg}, we conduct an ablation study to evaluate the impact of each component within the VFM-PLG module. The second row denotes the baseline performance, where the model is trained using pseudo labels generated from click annotations and the SAM. When a clustering algorithm is introduced to refine the pseudo label, the mAP improves substantially by 14.83\%. Additionally, applying the DAM to handle composite categories, such as cyclists, can further improve performance by 5.82\% AP. When geometric constraints are incorporated, the mAP reaches 47.37\%, surpassing methods that utilize 2D boxes as prompts. Combining these methods not only improves segmentation performance but also significantly reduces annotation costs, demonstrating the efficiency and practicality of our approach in weakly supervised 3D instance segmentation.


\begin{table}[ht]
    \centering
    \adjustbox{max width=0.55\linewidth}{
    \begin{tabular}{ccc} 
    \toprule
    Frames & mAP            & mIoU             \\ 
    \hline
    0      & 47.37          & 72.189           \\ 
    \hline
    1      & 47.52          & 68.346           \\
    2\cellcolor{lightgray}      & \textbf{52.18}\cellcolor{lightgray} & \textbf{74.449}\cellcolor{lightgray}  \\
    3      & 51.07          & 74.107           \\
    5      & 48.17          & 72.345           \\
    \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Ablation Study of the Number of Adjacent Frames.}}
    \label{tab:tsu1}
\end{table}

\begin{table}[ht]
    \centering
    \adjustbox{max width=0.9\linewidth}{
    \begin{tabular}{cccccc} 
    \toprule
    \multirow{2}{*}{Frames} & \multirow{2}{*}{Vote Mode} & \multicolumn{2}{c}{Dynamic} & \multirow{2}{*}{mAP} & \multirow{2}{*}{mIoU}  \\ 
    \cline{3-4}
                            &                            & Count        & Score        &                      &                        \\ 
    \hline
    0                       & $\mbox{-}$                 & $\mbox{-}$   & $\mbox{-}$   & 47.37                & 72.189                 \\ 
    \hline
    \multirow{5}{*}{2}      & \multirow{2}{*}{Hard}      & $\mbox{-}$   & $\mbox{-}$   & 48.54                & 73.138                 \\
                            &                            & $\checkmark$ & $\mbox{-}$   & 48.68                & 73.215                 \\ 
    \cline{2-6}
                            & \multirow{3}{*}{Soft}      & $\mbox{-}$   & $\mbox{-}$   & 49.97                & 73.152                 \\
                            &                            & $\checkmark$ & $\mbox{-}$   & 50.83                & 73.564                 \\
                            &                            & $\checkmark$\cellcolor{lightgray} & $\checkmark$\cellcolor{lightgray} & \textbf{52.18}\cellcolor{lightgray}       & \textbf{74.449}\cellcolor{lightgray}        \\
    \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Ablation Study of Voting Strategy in the TSU Module.} \textit{Hard} voting means that the predicted label of the majority class among the points within a voxel is selected as the updated label. In contrast, \textit{Soft} voting assigns the updated label based on the class with the highest average confidence score across all points within the voxel. \textit{Count} and \textit{Score} represent the use of dynamic thresholds, \textit{Count} dynamically adjusts the required number of votes, while \textit{Score} dynamically adjusts the confidence score threshold for label updates.}
    % These strategies aim to optimize label reliability based on the varying density of LiDAR point clouds.
    \label{tab:tsu2}
    \vspace{-2mm}
\end{table}

\noindent\textbf{Effect of the TSU.}
% 表格3和表格4提供了我们TSU模块的消融实验。在表格3中，我们可以看到在一定帧数范围内，随着帧数的增多，性能有提升，当使用2帧生成的结果进行更新时，达到最大性能52.18%mAP和74.449%mIoU。当帧数超过3帧时，动态目标移动过大，进步使得投票出现错误，导致性能下降。在表格4中，我们提供了多种不同投票策略的性能对比。当使用Hard投票方式时，第三行对比baseline（第一行），实例分割和语义分割性能分别提升1.17%mAP和0.949%mIoU，性能提升有限。当仅仅使用Soft投票方式时，性能提升2.6%mAP和0.363%mIoU。当配合我们提出的Distance-based reliability update strategy，性能提升明显，实例分割和语义分割性能分别提升4.81%mAP和2.26%mIoU。证明我们基于LiDAR点云近密远疏特性提出的更新策略的有效性。
Tables \ref{tab:tsu1} and \ref{tab:tsu2} provide the ablation studies for the proposed TSU module. In Table \ref{tab:tsu1}, we analyze the impact of using different numbers of frames for label updates. We observe a steady improvement in performance as the number of frames increases up to a certain point. Specifically, when updating labels using predictions from two adjacent frames, the method achieves its best performance, with 52.18\% mAP for instance segmentation and 74.449\% mIoU for semantic segmentation. However, as the number of frames exceeds three, the increased motion of dynamic objects causes greater discrepancies between frames, leading to erroneous votes and a consequent drop in overall performance.

Table \ref{tab:tsu2} compares several voting strategies to assess their impact on segmentation results. When employing the hard voting method (row 3), compared to the baseline method (row 1), we observe only modest improvements, with gains of 1.17\% mAP and 0.949\% mIoU. This limited improvement suggests that the hard voting is not sufficiently robust to handle noise in the predictions. In contrast, when applying the soft voting method (row 4), the performance improvement is more pronounced, yielding 2.6\% mAP and 0.963\% mIoU gains.

Furthermore, when we integrate our distance-based reliability update strategy (row 6), which adapts to the varying density of LiDAR point clouds based on their proximity to the sensor, we observe a significant increase in performance. Specifically, instance segmentation improves by 4.81\% mAP, while semantic segmentation sees a gain of 2.260\% mIoU. These results highlight the robustness of our proposed strategy in leveraging the inherent properties of LiDAR point clouds, particularly the denser distribution of points near the sensor and the sparser distribution at greater distances, to enhance the reliability of pseudo labels during training. This approach not only improves segmentation accuracy but also addresses challenges posed by noisy or uncertain predictions.

% Hard表示在投票时，将落在该体素中类别数量最多的点的预测标签作为更新标签，Soft表示将落在该体素中置信度平均得分最大类别的预测标签作为更新标签。Count和Score分别表示使用动态的投票数阈值和动态的置信度阈值。

\noindent\textbf{Effect of the manual annotation error.}
% Manual annotation 
% 为了模拟在手工标注过程中的误差，我们设置了不同click标注范围的扰动实验，如表格6所示。
% 表格第一列的值表示在bev视角下以实例中心为圆心，click range为半径的园内随机选择点作为click标注，其中0.0表示距离实例中心最近的点。
To simulate potential errors that may arise during manual annotation, we conduct experiments with varying click annotation ranges, as detailed in Table \ref{tab:click}. These results demonstrate that our method exhibits strong stability across different annotation ranges. Notably, even as the click range expands to 0.5 meters, there is no significant drop in performance, with both mAP and mIoU remaining well within acceptable limits. This robustness indicates that our approach is resilient to variations in the click annotation radius, consistently maintaining high performance regardless of the distance from the instance center. Such stability is crucial in real-world applications, where manual annotations can introduce variability, yet reliable segmentation results are still required.
\begin{table}[t]
    \centering
    \adjustbox{max width=0.6\linewidth}{
    \begin{tabular}{ccc}
    \toprule
    Error Range (m) & mAP            & mIoU             \\ 
    \hline
    0.0         & \textbf{55.35} & 74.770           \\
    \hline
    0.1         & 54.86          & 75.688           \\
    0.2         & 54.98          & 75.591           \\
    0.3         & 54.39          & \textbf{75.936}  \\
    0.5         & 54.76          & 74.444           \\
    \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Ablation Study of the Manual Annotation Error.} The first column of the table presents the click error range during manual annotation. Single click annotations are randomly selected from a circular region centered at the instance's center in the BEV plane, with the \textit{Error Range} defining the radius. A value of 0.0 indicates that the point closest to the instance center is selected.}
    \label{tab:click}
\end{table}

\noindent\textbf{Fine-tuning with our method.}
% Following the MWSIS, 我们将在我们YoCo框架下训练好的网络在不同比例的全监督数据上进行微调。当仅使用0.8%的数据进行微调，已经取得与全监督相同的性能（59.27% vs 59.26%）。当使用5%的数据进行微调时，已经超过了基于PTv3网络的全监督性能。这表明，在我们的框架下仅使用极少的数据即可达到与全监督相当的性能，大大降低了标注的成本，对比更加复杂的point-based网络，我们的方法还更具效率。
Following the ~\cite{jiang2024mwsis}, we fine-tune the trained network within our YoCo framework across different proportions of fully supervised data. As shown in Figure \ref{fig:finetune}, fine-tuning with a mere 0.8\% of the fully supervised data yields performance results nearly indistinguishable from those achieved under full supervision (59.27\% vs. 59.26\%). Moreover, when increasing the fully supervised data utilization to 5\%, our approach surpasses the fully supervised performance of the PTv3 network.

% The above experiments show that under our YoCo framework, this greatly reduces annotation costs and provides higher training efficiency compared to more complex point-based networks.

The above experiments demonstrate that our YoCo framework achieves performance comparable to fully supervised methods using only a minimal amount of annotations, significantly reducing annotation costs.
% In comparison to more complex point-based networks, our method is more efficient.
% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\linewidth]{img/finetune.pdf}
%     \caption{\textbf{3D Instance Segmentation Performance Comparison.} The weakly supervised training backbone for fine-tuning compared to the fully supervised performance.}
%     \label{fig:finetune}
% \end{figure}

